Uni-SMART: Universal Science Multimodal Analysis and Research Transformer

In scientific research and its application, scientific literature analysis is crucial as it allows researchers to build on the work of others. However, the fast growth of scientific knowledge has led to a massive increase in scholarly articles, making in-depth literature analysis increasingly challenging and time-consuming. The emergence of Large Language Models (LLMs) has offered a new way to address this challenge. Known for their strong abilities in summarizing texts, LLMs are seen as a potential tool to improve the analysis of scientific literature. However, existing LLMs have their own limits. Scientific literature often includes a wide range of multimodal elements, such as tables, charts, and molecule, which are hard for text-focused LLMs to understand and analyze. This issue points to the urgent need for new solutions that can fully understand and analyze multimodal content in scientific literature. To answer this demand, we present \textbf{Uni-SMART} (Universal Science Multimodal Analysis and Research Transformer), an innovative model designed for in-depth understanding of multimodal scientific literature. Through rigorous quantitative evaluation across several domains, Uni-SMART demonstrates superior performance over other text-focused LLMs. Furthermore, our exploration extends to practical applications, including patent infringement detection and nuanced analysis of charts. These applications not only highlight Uni-SMART's adaptability but also its potential to revolutionize how we interact with scientific literature.

==> backups/1_introduction.tex <==
\section{Introduction}
\textbf{Background.}
Scientific literature, encompassing patents and academic papers, is a treasure trove of valuable data, including but not limited to drug properties and activities, reaction pathways, manufacturing processes, and omics relationships. 
The extraction of this data, however, is notoriously labor-intensive and time-consuming. 
It requires meticulous manual reading, analysis, and extraction, processes that are not only slow but also prone to human error \cite{hong2021challenges, nasar2018information}.
Existing non-heuristic databases such as Sci-Finder and Reaxys rely heavily on human experts to perform these extractions. 
While they are effective in supporting certain types of data retrieval, such as chemical reactions, they lack the capacity for automatic extraction from newly published documents. 
This limitation poses a significant bottleneck in the timely utilization of scientific data, impeding research progress and the rapid application of new discoveries.
Thus, researchers and practitioners are in need of an intelligent navigator that can swiftly guide through the complexities of latest scientific data, identify relevant information with precision, and present it in a digestible format.

\textbf{Advent of LLMs.}
The advent of large language models (LLMs) such as ChatGPT has heralded a new era of natural language processing, demonstrating remarkable proficiency in a myriad of natural language tasks \cite{ouyang2022training, achiam2023gpt}. 
There has been a proliferation of literature assistance tools based on such models, like ChatPDF, which facilitate the extraction of text from PDF documents and engage in natural language question-answering. 
However, these tools are tailored predominantly for text extraction, and while they excel in processing and generating human-like text, they falter when confronted with the multimodal nature of scientific literature.
Scientific documents are replete with multimodal information that extends beyond text, including but not limited to statistical tables, molecule graphs, and chemical reactions. 
The extraction and interpretation of such multimodal data require an understanding that transcends textual information and delves into the realm of visual and structural data representation. 

\textbf{Briefs of Uni-SMART.}
To address these challenges, we have developed Uni-SMART (Universal Science Multimodal Analysis and Research Transformer), which extends the capabilities of LLMs beyond text, allowing for the interpretation of the rich visual and structural information that is paramount in scientific documentation. 
Uni-SMART is designed to recognize and interpret complex visual data such as charts, graphs, and molecular structures, alongside textual content, facilitating a comprehensive understanding of scientific materials.
This innovative approach not only augments the automated and precise data extraction process but also enriches the interaction between researchers and the vast expanse of scientific knowledge, paving the way for a more holistic and efficient research methodology.

\textbf{Evaluation of Uni-SMART.}
To rigorously assess the multimodal capabilities of Uni-SMART, a comparative analysis was conducted against existing heuristic literature analysis tools, which are mostly based on LLMs.
The tools included for comparison were ChatPDF, Claude, and GPT-4 \GL{Only GPT-4 now}. 
Our evaluation focused on extensive functionalities crucial for scientific research: table information extraction, molecular formula recognition, Markush structure recognition, synonyms/IUPAC understanding, chart understanding, reaction equation recognition, multimodal understanding, multimodal reasoning, text understanding, and textual reasoning.
The results demonstrated Uni-SMART's superior performance in all tested areas, especially in understanding and analyzing complex multimodal information, thus confirming its effectiveness as a tool for scientific literature analysis.

\textbf{Outlines of this report.}
In the following sections, we first provide an overview of the Uni-SMART model architecture, detailing its unique integration of visual and textual data processing capabilities in Section 2, Method. Section 3, Evaluation, presents detailed comparisons of Uni-SMART with other contemporary LLM-based approaches across a variety of tasks, showcasing its advanced capabilities in multimodal data interpretation. Section 4, Limitations and Future Directions, acknowledges the limitations of the current model and outlines future directions for enhancing its performance and broadening its application in scientific research. Finally, Section 5, Discussion and Conclusion, reflects on the broader implications of Uni-SMART's capabilities for scientific research, highlighting its potential to significantly enhance how scientists interact with and analyze scientific literature, thereby underlining the innovative impact Uni-SMART is poised to have on the field.

==> backups/3_evaluation.tex <==
\section{Evaluation}
\label{sec:eval}
% Including quantitative results and case studies.

In this section, we conduct a comprehensive evaluation of Uni-SMART's capabilities, covering a broad range of practical application domains, including general chemistry, photoelectric molecules, alloys, organic electrolytes, and biomedicine. \LZ{BDA should be explained if presented here, but I think it is not necessary to present it here. We could consider simply listing the names appearing in the subsections (like general chemistry, alloy materials, etc.) after they are converged.}

Table \ref{tab:statistical-overview} provides a statistical breakdown of the dataset. Each question within the dataset is accompanied by the necessary context, the current query, and the correct answer. Given our primary focus on reading comprehension within scientific literature, the context is predominantly provided in the form of documents (PDFs). This structure is designed to mimic the real-world process of extracting and understanding information from scientific texts, thereby facilitating a more authentic assessment of the model's capability in navigating and interpreting complex scientific content.
To ensure the highest level of accuracy and reliability in our dataset, we have engaged domain experts to perform multiple cross-verification checks on the test dataset, thereby confirming the correctness of the dataset labels.

\begin{table*}[htb]
\centering
\begin{tabular}{llll}
\toprule
Domain & \# of Tasks & Types of Questions & \# of Questions \\
\midrule
General Chemistry & & & \\
Organic Photoelectric Materials & & & \\
Organic Electrolytes & & & \\
Alloy Materials & 4 & Table Extraction, Single Choice, True/False & 175 \\
Drug Discovery & & & \\
Biomedicine & & & \\
\bottomrule
\end{tabular}
\caption{Statistical Overview of the Dataset.\GL{Update this table}}
\label{tab:statistical-overview}
\end{table*}


We conducted a comparative analysis through API calls with OpenAI's ChatGPT (version info) and GPT-4 (version info), both of which have demonstrated strong multimodal capabilities.
In addition to these, we also examined Anthropic's Claude (version info), a model that is often considered to be on par with ChatGPT in terms of performance.\GL{Update this}


% \textcolor{orange}{Baseline Setting Information}

\begin{itemize}
    \item GPT-4: Our API mimics the process of chatting with GPT-4 at \href{https://chat.openai.com}{https://chat.openai.com},  which is augmented with DALL-E, code interpreter and retrieval abilities.
    \item Claude: We developed an automated retrieval procedure of using API from \href{https://claude.ai}{https://claude.ai}, which mimics the process of chatting with Claude on the website with attached files. The API is slightly modified from \href{https://github.com/st1vms/unofficial-claude2-api}{https://github.com/st1vms/unofficial-claude2-api} to keep in consistency with the newest website version. \GL{remove this}
    \item Zero-shot COT: Chain-of-thought is implemented in a two-step manner. For any chat prompt, the first step is COT reasoning, for example: \GL{remove this}
\begin{lstlisting}
System: You are ChemistGPT, can help user insert substituents into markush formula to get SMILES formula (removing Hs). For example, if user's input is "*CCCC* |$R1_p;;;;;R2_p$|, R1 = OMe, R2 = NH2", you will reply the completed SMILES: "COCCCCN", without explanation. If you can't answer the completion, just reply "Unknown".

User: *C(*)CC(*)CC* |$A;;Pol_p;;;Q_e;;;M_p$|, A = H, Pol = NH2, Q = OH, M = OLi

**Assistant: Before answering, reason in a step-by-step manner as to get the right answer, then conclude with the answer.**

Assistant:
\end{lstlisting}
The second step is COT extraction:

\begin{lstlisting}
System: You are ChemistGPT, can help user insert substituents into markush formula to get SMILES formula (removing Hs). For example, if user's input is "*CCCC* |$R1_p;;;;;R2_p$|, R1 = OMe, R2 = NH2", you will reply the completed SMILES: "COCCCCN", without explanation. If you can't answer the completion, just reply "Unknown".

User: *C(*)CC(*)CC* |$A;;Pol_p;;;Q_e;;;M_p$|, A = H, Pol = NH2, Q = OH, M = OLi

Assistant: Before answering, reason in a step-by-step manner as to get the right answer, then conclude with the answer.

Assistant: <Answer from LLM>

Assistant: Given the above reasoning, the answer in the format requested by the question is:

Assistant:
\end{lstlisting}
\end{itemize}

\subsection{General Chemistry}

% Why these tasks

The "General Chemistry" evaluation set is a comprehensive suite of tasks designed to assess the capabilities of Large Language Models (LLMs) across a range of chemistry-related skills, from foundational knowledge to applied problem-solving and research analysis. This set encompasses four distinct tasks, each targeting different aspects of chemistry and scholarly comprehension. The inclusion of these tasks provides a holistic overview of an LLM's ability to engage with both the academic study of chemistry and the practical application of its principles. All test data are collected from OpenAI's \href{evals}{https://github.com/openai/evals} repository. An overview of the results is shown in table \ref{tab:quantitative-benckmarks-general-chemistry}.

% \textcolor{orange}{In each subsection, we include at least three major components: 
% \begin{itemize}
%     \item Quantitative benchmarks (\textit{e.g., } AP chemistry, Chemistry Competition with textbook ...), focusing on quantitative evaluation and improvement over baselines. Illustrated in Table \ref{tab:quantitative-benckmarks-general-chemistry}.
%     \item A comprehensive figure to show the metrics.
%     \item Comprehensive illustration (if needed). An impressive case to demonstrate Uni-SMART's abilities in this sub-area. Illustrated in Figure \ref{fig:icho}.
%     \item Details (which may be put in appendix finally). Including prompting methods, exam methodology, definition of metrics, etc.
% \end{itemize}
% }


\begin{table*}[htb]
\centering
\caption{Quantitative evaluation on general chemistry benchmarks.}
\begin{tabular}{cccccccc}
\toprule
Task                         & \#questions & Metric & \begin{tabular}[c]{@{}c@{}}Uni-SMART \\ \scriptsize{Evaluated Zero-shot} \end{tabular} & \begin{tabular}[c]{@{}c@{}}GPT-4 \\ \scriptsize{Evaluated Zero-shot} \end{tabular} \\
\midrule
MMLU College Chemistry       & 8   & Accuracy & \textbf{0.50} & 0.375 \\
Balancing Equations          & 100 & Accuracy & \textbf{0.45 $\pm$ 0.05} & 0.32 $\pm$ 0.05 \\
Abstract2Title               & 254 & Model-graded Score & 1.0 & 0.99 \\
Question Extraction          & 19 & Model-graded Score & \textbf{4.737} & 4.638 \\
\bottomrule
\end{tabular}
\label{tab:quantitative-benckmarks-general-chemistry}
\end{table*}



\begin{figure}
  \centering
  \includegraphics[width=0.8\columnwidth]{figures/metrics_example.png}
  \caption{Quantitative evaluation on general chemistry benchmarks. \textcolor{orange}{Example from GPT-4 report.} }
  \label{fig:quantitative-benckmarks}
\end{figure}

\subsubsection{MMLU College Chemistry}

MMLU (Massive Multitask Language Understanding) is a new benchmark designed to measure knowledge acquired during pretraining by evaluating models exclusively in zero-shot and few-shot settings. This makes the benchmark more challenging and more similar to how we evaluate humans. We select the \textbf{college chemistry} from its 57 subjects to examine the understanding of chemistry.

For each multiple-choice section, we used a zero-shot prompt to directly sample a multiple-choice answer letter and its choice content.

% The few-shot template (\emph{Now from GPT-4 tech report, later replaced by ours}) is shown in \ref{fig:few-shot}.

% \begin{figure}[H]
%   \centering
%   \includegraphics[width=0.8\columnwidth]{figures/few-shot_template.png}
%   \caption{Few-shot template for multiple-choice questions.}
%   \label{fig:few-shot}
% \end{figure}

\subsubsection{Balancing Equations}

The "Balancing Chemical Equations" evaluation task for Large Language Models (LLMs) is designed to assess the LLMs' ability to understand and apply principles of chemical stoichiometry and the laws of conservation of mass and energy. Balancing chemical equations is a fundamental skill in chemistry that involves adjusting the coefficients of the reactants and products in a chemical equation to ensure that the number of atoms for each element is the same on both sides of the equation, reflecting the conservation of matter.

This task not only tests the LLMs' capacity to parse and interpret the symbolic language of chemistry but also evaluates their problem-solving skills and their ability to engage with domain-specific knowledge. To successfully balance a chemical equation, an LLM must identify the reactants and products, understand the stoichiometric relationships between them, and apply mathematical reasoning to find a set of coefficients that balance the equation.

Since the newest version of GPT-4 can write the answer with code interpreter, we use chain-of-thought trick for GPT-4 to extract its final result.

\subsubsection{Abstract2Title}
\label{sec:abstract2title}

This evaluation benchmark tests the model's ability to generate a proper title using the abstract section of the literature.

The conciseness of the generated title is evaluated by GPT-4,  prompting like:

\begin{lstlisting}
You are assessing a submitted answer on a given task based on a criterion. Here is the data:
[BEGIN DATA]
***
[Task]: {input}
***
[Submission]: {completion}
***
[Criterion]: conciseness: Does the title properly describe the provided content?
***
[END DATA]
Does the submission meet the criterion? First, write out in a step by step manner your reasoning about the criterion to be sure that your conclusion is correct. Avoid simply stating the correct answers at the outset. Then print only the single character "Y" or "N" (without quotes or punctuation) on its own line corresponding to the correct answer. At the end, repeat just the letter again by itself on a new line.

    Reasoning:
% \end{lstlisting}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.8\columnwidth]{figures/comprehensive-illustrasion.jpeg}
%   \caption{Comprehensive illustration of general chemistry. \textcolor{orange}{Example from GPT-4V report.}}
%   \label{fig:comprehensive-illustration}
% \end{figure}

\subsubsection{Question Extraction}

The "Research Question Extraction" evaluation task for Large Language Models (LLMs) is aimed at assessing the models' ability to identify, extract, and summarize the primary research question or questions from a scientific paper's abstract. This task challenges the LLMs to demonstrate deep comprehension of the abstract's content, which is a concise summary that typically includes the background, purpose, methodology, results, and conclusions of the research. The primary goal is to distill this information into a clear, concise statement or set of statements that encapsulate the core research question(s) the paper seeks to address.

This evaluation task tests several key capabilities of LLMs, including their understanding of complex and domain-specific language, ability to discern the main focus amidst potentially broad and detailed information, and proficiency in summarizing and reformulating academic content. Research question extraction requires not just surface-level processing of the text but a deeper analysis to identify the research gaps the study aims to fill, the hypotheses it tests, or the problems it seeks to solve.

This task is particularly relevant for evaluating the utility of LLMs in academic and research settings, where efficiently understanding and extracting the essence of scholarly articles can aid in literature reviews, research proposal development, and the identification of research trends and gaps. It underscores the potential of LLMs to support researchers, scholars, and students by streamlining the process of engaging with the vast and ever-growing body of scientific literature.

The answers are evaluated by GPT-4 to give scores ranging from 1 to 5, similarly prompted to that in \ref{sec:abstract2title}.

\subsubsection{Conclusion}

From the above results, we can see that for tasks from foundational knowledge to applied problem-solving and research analysis, Uni-SMART performs better than the other universal large models. This indicates Uni-SMART's better understanding due to its multi-modal comprehension abilities.

% \subsection{Organic Photoelectric Materials}

% [Example]

\subsection{Organic Electrolytes}
Organic electrolytes are electrolytic solutions extensively used in battery technologies, especially in lithium-ion batteries. Comprising organic solvents, lithium salts, and additives when necessary, these electrolytes facilitate ion transfer within the battery, enabling energy storage and release. The composition and properties of organic electrolytes are crucial for battery performance, stability, and safety. Therefore, efficiently and accurately extracting information about electrolytes from the articles is crucial for researchers to conduct experiments.

In this chapter, we aim to evaluate Uni-SMART's semantic understanding of electrolyte-related information from two perspectives: solubility data and reaction equations. We mainly observed its capability in the task of table extraction, thereby demonstrating Uni-SMART's commendable retrieval effectiveness compared to other LLMs. All data mentioned in this chapter is obtained from open-source literature. The comparison of performance of models are shown in Table \ref{tab:solution_table}. To minimize the impact of random errors, we run five times with reported mean and stdev. We also utilized one shot chain of thought to enhance the model's performance.

\begin{table*}[h]
\centering
\begin{tabular}{cccccccc}
\toprule
Task &\#Literature &Metric  &\begin{tabular}[c]{@{}c@{}}Uni-SMART \\ \scriptsize{Zero-shot} \end{tabular} & \begin{tabular}[c]{@{}c@{}}GPT-4 \\ \scriptsize{Zero-shot} \end{tabular}\\
\midrule

&&Field Cov &\textbf{0.9500} $\pm$ 0.0612 &0.4500 $\pm$ 0.1000\\
&&Index Cov &\textbf{0.9500} $\pm$ 0.0612 &0.4500 $\pm$ 0.1000\\
Solubility data extraction &8
&Value Acc &\textbf{0.5888} $\pm$ 0.0255 &0.3021 $\pm$ 0.0754\\
&&Record Acc &\textbf{0.3736} $\pm$ 0.0216 &0.1614 $\pm$ 0.0554\\
&&Value Mat &\textbf{0.5888} $\pm$ 0.0255 &0.3021 $\pm$ 0.075\\
&&Record Mat &\textbf{0.3736} $\pm$ 0.0216 &0.1614 $\pm$ 0.0554\\
\midrule
&&Field Cov &\textbf{1.0000} $\pm$ 0 &0.6000 $\pm$ 0.4899\\
&&Index Cov &\textbf{1.0000} $\pm$ 0 &0.6000 $\pm$ 0.4899\\
Reaction data extraction &1
&Value Acc &\textbf{0.9139} $\pm$ 0.1438 &0.2650 $\pm$ 0.2171\\
&&Record Acc &\textbf{0.8640} $\pm$ 0.2269 &0.0698 $\pm$ 0.0637\\
&&Value Mat &\textbf{0.9139} $\pm$ 0.1438 &0.2650 $\pm$ 0.2171\\
&&Record Mat &\textbf{0.8640} $\pm$ 0.2269 &0.0698 $\pm$ 0.0637\\



\bottomrule
\end{tabular}
\caption{Quantitative evaluation on electrolyte information extraction benchmarks.}
\label{tab:solution_table}
\end{table*}



\subsubsection{Solubility data extraction}
In this task, we intend to investigate the Uni-SMART's capability in retrieving solubility-related tables. Considering the fact that papers related to the topic of solutions typically select data from various aspects to describe the system, requesting models combine multiple tables into an appropriate format for fuzzy matching turns out to be overly difficult. Therefore, we choose to focus more on examining the semantic understanding ability of LLMs, enabling the model to select the most relevant and largest table related to "solubility" from numerous alternatives, and then converting it into specified format.

We prompt the model with:
\begin{lstlisting}[literate={×}{{$\times$}}1 {±}{{$\pm$\ }}1 {°}{{$^\circ$}}1 {（）}{{()}}1]
You need to follow these steps to extract tables from the paper:
1. Find all tables which contains the word "solubility". If you cannot find anyone, then find all tables related to "solubility".
2. Select the table with most salts and solvents.
3. Collect all the headers of the table and generate a list.
4. If there's no "Compound"(Compound means salt or solute) and "Solvent" in the list, place them at the first two positions in the list. 
5. Output the whole table in csv format and satisfy these requirements:
    (1) Do not truncate tables using "...". Always output the complete tables.
    (2) Quote the values only if they contain commas.
    (3) Keep all the superscripts in the form like "^3", "^+" or "^a".
    (4) Do not use "NaN" to replace the blank cells, just leave it empty.
    (5) Use "x" to replace all "×", Use "()" to replace all "（）"
    (6) Always add space before and after operators like " ± ".
    Remember, the table format should be correct. Here is an example, the original table is:
    ```csv
    Table 1 solubilities (mole fraction x),,
    t/°C,NaCl,
    ,DMF,PC^b
    25,1.01 x 10^-2,8.3 x 10^-3
    15,1.25 x 10^-2,9.0 x 10^-3
    ,CaSO4^a,
    ,DMF,PC^b
    25,,5.6 x 10^-2
    15,1.83 x 10^-1,6.2 x 10^-2
    ```
    It should be converted to:
    ```csv
    Compound,Solvent,t/°C,solubilities (mole fraction x)
    NaCl,DMF,25,1.01 x 10^-2
    NaCl,DMF,15,1.25 x 10^-2
    NaCl,PC^b,25,8.3 x 10^-3
    NaCl,PC^b,15,9.0 x 10^-3
    CaSO4^a,DMF,25,
    CaSO4^a,DMF,15,1.83 x 10^-1
    CaSO4^a,PC^b,25,5.6 x 10^-2
    CaSO4^a,PC^b,15,6.2 x 10^-2
    ```
\end{lstlisting}

\subsubsection{Reaction data extraction}

In this task, we intend to examine Uni-SMART's ability to extract information about dissolution reaction equations. We ask the model to extract only those tables in the papers that are related to the reaction, simultaneously merge the content of these tables together, and finally convert them into proper format according to the requirements.
We prompt the model with:
\begin{lstlisting}[literate={×}{{$\times$}}1 {−}{{$-$}}1 {°}{{$^\circ$}}1]
While reading this paper, please summarize a complete list of the names and abbreviations of all reactions.
Then follow the below process step by step:
1. Find all the tables with relevant information.
2. Output the table in csv format. Here are some requirements you must satisfy:
    (1) You must preserve all the superscript in the form like "^3", "^a" or "^+".
    (2) The table headers must be strictly consistent with the original text. There's no need to add units like "temperature(°C)".
    (3) The first column should be renamed as "Compound".
    (4) Always add space before and after operators like " + ".
    (5) Use "-" to replace all "−".
    At the same time, here is an example:
    ```csv
    Compound,heat of solvation,temperature^a,density
    DMF + Na^+ = DMF-Na^+,101.5,25,0.78
    2EtOH + EtOH = 3EtOH,50.6,15,1.06
    ```
  3. If there are multiple tables, concat them. You should never truncate them, and should always give me the complete table.
\end{lstlisting}

\subsubsection{Conclusion}
The results in table \ref{tab:solution_table} demonstrate that Uni-SMART outperformed GPT-4 in these table extraction tasks. This confirms the model's superior semantic understanding of science related information such as electrolytes, as well as its ability to grasp the requirements of format details. Hence, we can expect this model to help more researchers through retrieval augmented generation.


\subsection{Alloy Materials}

Alloy materials are materials with metal characteristics that are mixed by two or more metal elements in a certain proportion, as shown in Figure \ref{fig:alloy}. Alloys are widely used in aerospace, automobile manufacturing, construction, electrical appliances and other fields. By adjusting the composition and preparation process, the alloy material can achieve specific properties and requirements \cite{caron1983improvement}. Therefore, it is very important to extract the alloy composition and process value from the literature for the design of the alloy.

\begin{figure}[H]
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/alloy.jpg}
  \caption{Alloy Heat Treatment Design.}
  \label{fig:alloy}
\end{figure}

In this chapter, we will investigate the capabilities of Uni-SMART in extracting information for alloy design. We have designed a comprehensive set of tasks related to literature research, including extraction of alloy composition, extraction of process values and determination of process sequence, as well as sample differentiation.
The standard answers for all tasks in this section are manually extracted and verified by another person. 1) In the composition extraction task, only part of the materials for each paper are prepared in the standard answer. Therefore, the extraction result of the large model should contain the standard answer, and the superfluous content should not be judged and counted. 2) The definition of the alloy process steps is based on the complete heat treatment process, such as the two consecutive process steps of annealing and tempering, each step contains the temperature rise, constant temperature and cooling stage. At this time, the previous process of tempering should be judged to be annealing, rather than annealing cooling.
Through our evaluation, we summarize the capabilities of different LLMs in alloy research as Table \ref{tab:alloy_res_table}. 
% The descriptions of alloying elements vary widely in these papers. Where available, the element content is listed in the table. Some literatures default to alloy names to reflect element content.



\begin{table*}[h]
\centering
\begin{tabular}{cccccccc}
\toprule
Task                         & \#Literature & Metric     & Uni-SMART \scriptsize{Zero-shot}& GPT-4 \scriptsize{Zero-shot}\\
\midrule
Composition Extraction    & 55   & Index Cov      & \textbf{0.948}       &  0.879         \\
                          &           & Field Cov      & \textbf{0.948}       &  0.879         \\
                          &           & Value Cov      & \textbf{0.415}       &  0.380         \\
Target Extraction         & 50   & Accuracy          & \textbf{0.820}       &  0.725          \\
Treatment Sequence        & 25  & Accuracy          & \textbf{0.833}      &  0.521         \\
Sample Differentiation    & 50   & Accuracy          & \textbf{0.790}       &  0.528          \\

\bottomrule
\end{tabular}
\caption{Quantitative evaluation on alloy discovery benchmarks.}
\label{tab:alloy_res_table}
\end{table*}

\subsubsection{Composition Extraction}

Extracting alloy composition information from the text or table of the article and unifying structured processing can help researchers make more effective use of historical data and provide experience guidance for subsequent design. This comprehensive task evaluates the LLMs' ability to extract alloy composition (containing all element content) for text and table. 
The extraction position of alloy elements typically falls into two cases: (1) The element content is stored in a table, as illustrated in the following Table \ref{tab:alloy_sample}; (2) The element content is implicitly indicated by the alloy name. For instance, 'Fe30Co20Ni50' represents an atomic ratio of 30\% Fe, 20\% Co, and 50\% Ni. The objective of this task is to comprehensively extract the aforementioned information and organize it into a resultant table while calculating the matching score between the standard answer table and the extraction result table. This showcases LLM's ability to integrate, extract, and structure multi-modal information \cite{kim2021prediction}.

% Dong–Cho Kim *, Tomo Ogura, Ryosuke Hamada, Shotaro Yamashita, Kazuyoshi Saida . Prediction of reversible α/γ phase transformation in multi-pass weld of Fe-Cr-Ni ternary alloy by phase-field method,  2021
% https://doi.org/10.1016/j.jajp.2021.100067


\begin{table*}[h]
\centering
\begin{tabular}{cccccccc}
\toprule 
AlloyName       & Composition & Composition    & Composition     & Composition    & Composition   & Composition  \\
\midrule
/               & C           & Cr             & Cu              & Fe             & Mn            & Mo           \\
\midrule
LeanDSS         & 0.014 \%    & 20.85 \%       & 0.09 \%         &  73.38 \%      & 1.49 \%       &   0.30 \%      \\
StandardDSS     & 0.012 \%    & 22.46 \%       & 0.17 \%         &  69.94 \%      & 1.81 \%       &   3.07 \%      \\
SuperDSS        & 0.013 \%    & 24.98 \%       & 0.20 \%         &  63.41 \%      & 0.48 \%       &   4.03 \%     \\
\bottomrule
\end{tabular}
\caption{Alloy composition example.}
\label{tab:alloy_sample}
\end{table*}

The metrics are defined as:

\begin{itemize}
    \item Field Cov: The percentage of matched column names to expected output table columns, such as "C", "Cr", "Cu" .etc;
    \item Index Cov: The percentage of matched compound names to expected output table;
    \item Value Acc: The percentage of correct values, indexed by alloy name and field name, where the value is matched by Levenshtein method\cite{2007Fast}.
\end{itemize}

We prompt the model with:

\begin{lstlisting}
"Prompt":
Please give a complete list of alloy names and compositions of all alloys in this paper.
If there is no alloy composition element ratio in the text, try to extract the element ratio from the alloy name from the perspective of alloy experts.
Output in one csv format with multiindex (2 header), The names in first header are 'AlloyName' and 'Composition' forcely. The names in the second header are element names of alloy.
Starting on the third row, list the alloy names and their corresponding element content. Based on the number of reference commas, the element name corresponds to the content.
Please write units not in header but in value like "50 wt.%", "30 at.%", "20 %" if with unit.
Such as the following example.
```csv
AlloyName, Composition, Composition, Composition       
nan, Fe, Co, Al       
Fe70Co15Al3, 70 %, 15 %, 3 %       
Fe70Co18, 70 %, 18 %,  nan, 
```
\end{lstlisting}

\subsubsection{Target Extraction}

The properties of the alloy are determined by the composition of the alloy and the process, which contains processing and heat treatment .etc. So the value of the extraction heat treatment is very critical. The task aims to determine the maximum temperature value for heat treatment of the alloy. To ensure accurate statistical analysis, single-choice questions have been employed in prompts. Consistency between the model-provided options and the standard answer indicates that the large-scale model effectively extracts crucial process-related information. 

Examples of process paragraphs \cite{villa2020physical}:
% Materials 2020, 13, 4806; doi:10.3390/ma13214806 www.mdpi.com/journal/materials
% Physical Characterization of Sintered NiMnGa
% Ferromagnetic Shape Memory Alloy
% Francesca Villa * , Adelaide Nespoli , Carlo Fanciulli, Francesca Passaretti and Elena Vill

\begin{lstlisting}
Raw text:
"Cast NiMnGa samples, of Ni50Mn30Ga20 nominal composition, were prepared by 5 arc melting cycles of the pure elements (electrolytic Ni 99.97%, electrolytic Mn 99.5% and Ga 99.99%) instoichiometric ratio, in a non-consumable electrode furnace (Leybold LK6/45) (Leybold, Cologne, Germany). As-cast ingot was ground to powder in a planetary ball mill (Fritsch Pulverisette 4) (FritschIdar-Oberstein, Germany) and the powder size selected by means of sieves. Densified pellets wereproduced by die pressing alloy powders with different average size (lower than 50 um or between 50 and 100 um) at 0.75 GPa at room temperature and sintered by a thermal treatment at 925 \circ C for 24, 72, and 168 h in an Ar atmosphere, followed by slow cooling in the furnace. Sintered pellets hadthe following dimensions: approximately 3 mm in height and 13 mm of diameter. Table 1 providesa summary of the prepared sintered samples."
\end{lstlisting}

We prompt the model with:

\begin{lstlisting}
"Prompt":
"Input": [{"role": "system", "content": "You are a highly intelligent alloy researcher who answers the following multiple choice question correctly.\nOnly write the answer down."}, {"role": "user", "content": "In the upper paper, what is the maximum temperature of the heat treatment process for all alloys?\n\na) 925 C\nb) 168 C\nc) 100 C\nd) 1025 C"}]

"Ideal": "c) 925 C"

"Answer": "c) 925 C"
\end{lstlisting}

The metrics are defined as:
\begin{itemize}
    \item Accuracy: The percentage of matched answer.
\end{itemize}

\subsubsection{Treatment Sequence}
Each process of alloy treatment has a clear sequence requirement, so it is necessary to ensure that the sequence of the extracted heat treatment process is consistent with the experimental sequence. For example, after solution treatment, the sample is further aged to ensure the internal gravitational release of the sample. This task aims to objectively analyze and evaluate the sequential relationship between two heat treatment and provide True/False answers. In addition, if a certain heat treatment name does not exist in paper, it should be considered False. This task assesses the LLM's logical ability to judge treatment order from text. 

The following are success case and failure case:

\begin{lstlisting}
1. Failure case:
"Prompt":
"Input": [{"role": "system", "content": "You are a highly intelligent alloy researcher who focus on heat treatment process (homogenization, annealing, aging, solution, quenching, tempering .etc) and answers the following question correctly./nOnly write the True or False."}, {"role": "user", "content": "In the upper paper, Is the processing heat treatment technique after the homogenization called aging?"}]

"Ideal": "True"

"Evaluate": "False"

2. Success case:
"Prompt":
"Input": [{"role": "system", "content": "You are a highly intelligent alloy researcher who focus on heat treatment process (homogenization, annealing, aging, solution, quenching, tempering .etc) and answers the following question correctly./nOnly write the True or False."}, {"role": "user", "content": "In the upper paper, Is the processing heat treatment technique before the HIP pressure called annealing?"}]

"Ideal": "False"

"Evaluate": "False"

 \end{lstlisting}

 The metrics are defined as:
\begin{itemize}
    \item Accuracy: The percentage of matched answer.
\end{itemize}


\subsubsection{Sample Differentiation}
Alloys with the same composition but treated by different processes are considered different samples because they have different properties. Therefore, the distinction between different samples needs to consider the difference in their processes. This task is designed to comprehensively judge the number of different alloy samples proposed or studied by the authors. The task mode is single-choice question. This comprehensive task assesses the logical ability of the LLMs to alloy distinctions from text.

The following example is process paragraphs where the sample are treated by different processes \cite{hernandez2017evaluation}:

% Hernández-Rivera JL, et al. Evaluation of hardening and softening behaviors in Zn–21Al–2Cu alloy processed
% by equal channel angular pressing. J Mater Res Technol. 2017. http://dx.doi.org/10.1016/j.jmrt.2017.06.006

\begin{lstlisting}
Raw text:
"An induction furnace was used to produce the Zn-21A1-2Cu alloy by melting proper amounts of Zn (99.99%), Al (99.99%)and Cu (99.96%). The alloy was melted in a graphite crucibleexposed to air and poured into cylindrical bars of 19 mm indiameter and 35 mm in length. After that, some bars were homogenized at 350 \circ C for 24h in air. Cast and homogenized samples were subjected to an equal channel angular extrusion(ECAP) in a die with two cylindrical channels with a diameter of 15.8mm.The innerintersectingangle (y) was 90\circ and the outerangle (y) was 36\circ. All samples were extruded by two and sixpasses with a ram velocity of 5 mm/min and by using B. route.The lubricant used was MoS, and it was applied to both chan.nels on each pass. "
 \end{lstlisting}

We prompt the model with:

\begin{lstlisting}
"Prompt":
"Input": [{"role": "system", "content": "You are a highly intelligent alloy researcher who answers the following multiple choice question correctly.\nOnly write the answer down."}, {"role": "user", "content": "Materials with the same components but processed through different techniques are considered as different alloys because they possess distinct properties. In the upper paper, please provide a count of all the alloys proposed and discussed by the authors?\n\na) 3\nb) 0\nc) 2\nd) 1"}]

"Ideal": "d) 2"
 
\end{lstlisting}

The metrics are defined as:
\begin{itemize}
    \item Accuracy: The percentage of matched answer.
\end{itemize}


\subsubsection{Conclusion}

From the above results, we can see that for most tasks the Uni-SMART which makes reasonable use of multi-modal information, performs better than the other universal large models.

(1) For information extraction with fixed field names, such as directly specifying the name of the element to be extracted, the large model can basically achieve very high extraction accuracy (Uni-SMART/0.948, GPT-4/0.879). In terms of the matching of element values, Uni-SMART showed a better matching degree (0.415) than GPT-4. But Neither model is satisfactory, which is related to the excessive redundant Synonyms information, resulting in a mismatch between the alloy name and values. The use of more stringent queries may lead to further improvements in value accuracy.

(2) For treatment sequence and sample differentiation tasks, the accuracy of Uni-SMART is about 0.30 higher than that of GPT-4. Uni-SMART's more reasonable identification and placement for paper of  double-column structure may be the reason for its higher accuracy. Therefore, for problems that require logical judgment, the accurate analysis of the article structure is very important. simple numerical extraction task is not sensitive to article structure.

In a word, future extraction queries in the custom alloy field, as well as stricter format restrictions on results, may be the key to fully leveraging the information extraction capabilities of large models.

\subsection{Polymer Materials}
In this chapter, we evaluate the efficacy of Uni-SMART in extracting crucial attributes associated with polymer materials from scientific literature. We specifically focus on the use of conjugated polymers in organic solar cells as case studies, extracting vital values from the literature, including PCE, Voc, and other electronic properties. By employing LLM to extract these properties, we demonstrate significant potential for the AI community in polymer modeling, such as computer-aided screening, targeted design, and optimization. To ensure robust testing, we run five times with reported mean and stdev.

We summarize the results as follows:
\begin{table*}[h]
\centering
\begin{tabular}{cccccccc}
\toprule
Task & \#Literature & Metric & Uni-SMART \scriptsize{Zero-shot} & GPT-4 \scriptsize{Zero-shot} & Claude \scriptsize{Zero-shot} \\
\midrule
Property Extraction & 15 & \begin{tabular}{c} Field Cov \\ Index Cov \\ Value Acc \\ Record Acc \\ Value Mat \\ Record Mat \end{tabular} & \begin{tabular}{c} \textbf{1.0} $\pm$ 0.0 \\ \textbf{1.0} $\pm$ 0.0 \\ \textbf{0.8644} $\pm$  0.0307 \\ \textbf{0.7280} $\pm$ 0.0412 \\ \textbf{0.8644} $\pm$  0.0307 \\ \textbf{0.7280} $\pm$ 0.0412 \\ \end{tabular} & \begin{tabular}{c} 0.8533  $\pm$ 0.0499 \\ 0.8533 $\pm$ 0.0499 \\ 0.7619 $\pm$ 0.0294 \\ 0.6389 $\pm$ 0.0383 \\ 0.7619 $\pm$ 0.0294 \\ 0.6389 $\pm$ 0.0383 
 \end{tabular}  & \begin{tabular}{c} / \\ / \\ / \\ / \\ / \\ / \end{tabular} \\
\bottomrule
\end{tabular}
\caption{Quantitative evaluation on polymer extraction benchmarks.}
\label{tab:polymer extract}
\end{table*}

We prompt the model with:

\begin{lstlisting}
"Prompt":
Please give a complete list of Nickname, PCE_max(%), PCE_ave(%), Voc (V), Jsc (mA cm^2), FF;
* Output in csv format with columns of those attribution, do not write units only the value like "10.5".
* If there are multiple tables, concat them. Don't give me reference or using "...", give me complete table!
* Should return all columns mentioned, if empty just return `NaN`. Nickname should not be empty.
* Nickname should be short name of polymers, for example: `PCBM:PffBT4T-2OD:PC61PM` should return `PffBT4T-2OD`.
* Only return acceptor `PC71BM` related records.
* If with different experiment settings for the same nickname, only return the record with `highest PCE` !
* Should find more information from the whole content, including tables, text.
* For FF use 0.xx instead of xx.x, for example: 63.0 should return 0.63 !
for example, you should return:
```csv
Nickname,PCE_max(%),PCE_ave(%),Voc (V),Jsc (mA cm^2),FF
PBTTT-C14,2.34,2.34,0.53,9.37,0.48
```
\end{lstlisting}

From the above results, we can see that for most tasks the Uni-SMART which makes reasonable use of multi-modal information, performs better than the other universal large models. 

\subsection{Drug Discovery}

In this chapter, we examine Uni-SMART's capabilities in the realm of drug discovery. We devise a comprehensive set of tasks related to \emph{patent and literature research}, ranging from affinity data extraction, enzyme data extraction and patent coverage.

Through our evaluation, we summarize the capabilities of Uni-SMART in drug discovery as follows:



\begin{table*}[h]
\caption{Quantitative evaluation on drug discovery benchmarks.}
\label{tab:quantitative-benckmarks-drug-discovery}
\centering
\begin{tabular}{cccccccc}
\toprule
Task                         & \#questions & Metric & Uni-SMART & GPT-4  \\
\midrule
Affinity Data Extraction     & 10 pdfs & \begin{tabular}[c]{@{}c@{}} \\ Field Cov \\ Index (Compound Name) Cov \\ Value Acc \\ Record Acc \\ \begin{equation*}\quad\end{equation*} \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{1.00} \\ \textbf{1.00} \\ \textbf{0.417} \\\textbf{0.417} \end{tabular} & \begin{tabular}[c]{@{}c@{}}0.89 \\ 0.89 \\ 0.274 \\ 0.274 \end{tabular}  & \\
% Markush2Molecule             & 20      & Accuracy                    & 0.0  &  0.0   \\
% Tag2Molecule                 & 50 in 10 pdfs & Accuracy              & 0.0  &  0.0   \\
Molecule in Document         & 4 in 4 pdfs & Accuracy              & \textbf{0.75} &  0.0   \\
Target Extraction            & 10 pdfs & Model-graded Matching Score & 0.8  &  0.8   \\
Enzyme Data Extraction       & 10 pdfs & Accuracy & /    &       &      \\
\bottomrule
\end{tabular}
\end{table*}

\subsubsection{Affinity Data Extraction}

This comprehensive task evaluates the LLM's ability to extract affinity table (containing molecules' tags, SMILES, and affinity to different targets in bioassays). This evaluation task tests several key capabilities of LLMs, including their understanding of complex and domain-specific language, and understanding of molecules and tables. Affinity data extraction requires not just surface-level processing of the text but a deeper analysis to match different modalities.

For an example output, 

\begin{table}[htb]
\caption{Example output of affinity data extraction task}
\begin{tabular}{ccccccc}
\hline
Compound & Name    & SMILES                & \multicolumn{2}{c}{Affinities}                                      \\
         &         &                       & Cytotoxicity in 2.2.15 Cells (IC50) & Anti-HBV Activity in 2.2.15 Cells (EC50) \\ \hline
1       & / & C1[C@H](O[C@H]([C@H]1F)N2C=NC3=C(N=CN=C32)N)CO & >200000 nM & >10000 nM \\
2       & / & C1[C@H](O[C@H]([C@H]1F)N2C=CC(=NC2=O)N)CO & >200000 nM & 4000 nM \\ 
3       & / & CC1=CN(C(=O)NC1=O)[C@H]2C[C@@H]([C@H](O2)CO)N=[N+]=[N-] & NA & NA \\
\hline
\end{tabular}
\end{table}

the metrics are defined as:

\begin{itemize}
    \item Field Accuracy: The percentage of fuzzy-matched column names to expected output table columns;
    \item Compound Accuracy: The percentage of matched compound names to expected output table;
    \item SMILES Accuracy: The percentage of correct SMILES, indexed by compound name;
    \item Value Accuracy: The percentage of correct values, indexed by compound name and field name.
\end{itemize}

We prompt the model with:

\begin{lstlisting}
You are an expert in the field of pharmaceutical chemistry, and your task is to summarize the results of activity assays from an article in a tabular format. Please follow these steps to complete the task:

1. Determine if the article includes an activity assay. If it does, locate the section(s) presenting the assay results, which are usually in one or more tables.
2. Compile all the activity assay results into a single table. You may use multiple columns to represent different conditions or outcomes of various experiments.
3. Identify the names or codes used in the table, such as Example 1 or Compound A, and find the corresponding sections in the article that mention these substances. Extract the full name and SMILES notation of each substance.
4. Compile the names and SMILES notations of each substance in the table. Output in csv format with multiindex (Affinities, protein/cell line), write units not in header but in the value like "10.5 µM". Quote the value if it has comma! For example:
```csv
Compound,Name,SMILES,Affinities,Affinities,Affinities,Affinities
,,,5HT1A (IC50),5HT1D (IC50),5HT-UT (IC50),5HT1E (<affinity type>)
"5a","Aspirin","CC(=O)Oc1ccccc1C(=O)O",2.0 nM,8.0 nM,12.6 nM,>1000 nM
```
5. If there are multiple tables, concat them. Don't give me reference or using "...", give me complete table!
\end{lstlisting}

A detailed example is shown in table \ref{table:patent2}.

The dataset is curated from PubChem BioAssays [ link ] to cover literature from different journals and years. Since the original dataset is organized by Bioassay numbers, we merge the source data according to their DOIs, and carefully select 10 papers from these DOIs. The papers have a large coverage of protein targets and cell lines, in the meanwhile have different display formats of the tables.

% \begin{itemize}
%     \item All chemical structures in the table;
%     \item Tagging all the molecules in the context and show the tags in the table;
%     \item Showing a Markush formula above the table and list the substituents in the table
% \end{itemize}

In the following subsections, we divide the affinity table extraction task logically, into several direct sub-tasks. 

% \subsubsection{Markush2Molecule}

% This task evaluates the model's ability to get correct SMILES given Markush formula (in CXSMILES pattern) and substituents.

% \begin{lstlisting}
% System: You are ChemistGPT, can help user insert substituents into markush formula to get SMILES formula (removing Hs). For example, if user's input is "*CCCC* |$R1_p;;;;;R2_p$|, R1 = OMe, R2 = NH2", you will reply the completed SMILES: "COCCCCN", without explanation. If you can't answer the completion, just reply "Unknown"
% User: *C(*)CC(*)CC* |$A;;Pol_p;;;Q_e;;;M_p$|, A = H, Pol = NH2, Q = OH, M = OLi
% Assistant: 
% \end{lstlisting}

% \subsubsection{Tag2Molecule}

% This task evaluates the model's ability to find correct SMILES given its tag in a document.

% \begin{lstlisting}
% System: You are ChemistGPT, can help user get SMILES formula from documents. Give me only the answer without explanation. If you can't answer the completion, just reply "Unknown"
% User: What's the SMILES formula of molecule "Sumatriptan"?
% Assistant: 
% \end{lstlisting}

\subsubsection{Molecule in Document}

This comprehensive task evaluates the model's ability to judge whether the molecule (represented by SMILES) is covered in a document. A detailed example is shown in table \ref{table:patent}.

\subsubsection{Target Extraction}

This task evaluates the model's ability to find all related targets (protein / cell line) of the bioassays given a document. The extracted targets are compared to ideal answers by asking GPT-4:

\begin{lstlisting}
You are comparing a submitted answer to an expert answer on a given question. Here is the data:

[BEGIN DATA]
************
[Question]: Please show which targets (protein / cell line) this paper's experiments do against. 
************
[Expert]: {ideal}
************
[Submission]: {completion}
************
[END DATA]

Compare the factual content of the submitted answer with the expert answer. Ignore any differences in style, grammar, or punctuation.
The submitted answer may either be a subset or superset of the expert answer, or it may conflict with it. Determine which case applies. Answer the question by selecting one of the following options:
    (A) The submitted answer is a subset of the expert answer and is fully consistent with it.
    (B) The submitted answer is a superset of the expert answer and is fully consistent with it.
    (C) The submitted answer contains all the same details as the expert answer.
    (D) There is a disagreement between the submitted answer and the expert answer.
    (E) The answers differ, but these differences don't matter from the perspective of factuality.
\end{lstlisting}

Then the answer is given a score according to the model-selected choice: 0.5 for \textbf{A}, 0.75 for \textbf{B}, 1.0 for \textbf{C}, 0.0 for \textbf{D}, and 0.75 for \textbf{E}.

\subsubsection{Enzyme Data Extraction}
This comprehensive task evaluates the capability of LLM's to extract enzyme-related parameters, including molecular tags, SMILES (Simplified Molecular Input Line Entry System), Km (Michaelis constant), pH range, inhibitor names, sites of action, substrates,  organism and comment. For an example output, 

\begin{tabular}{ccccccc}
\hline
\parbox[t]{2cm}{Activating\\Compound} & Substrate & Inhibitor & Km & Comment & Localization & Organism   \\
\hline
 Cu2+ & - & - & - & 0.01 mM, slight activation  & - & Bos taurus \\ 
 - & - & NH4+ & - & 2 mM & - & Homo sapiens \\ 
 - & - & - & - & - & periplasm & Bos taurus \\
 - & NADPH & benzaldehyde & 0.12 mM & enzyme form ATP & - & Bos taurus \\
\hline
\end{tabular}

the metrics are defined as:
\begin{itemize}
    \item Field Accuracy: The percentage of fuzzy-matched column names to expected output table columns;
    \item Activating Accuracy: The percentage of matched activating compound and inhibitor to expected output table;
    \item Substrate Accuracy: The percentage of matched substrate, indexed by substrate;
    \item Km Accuracy: The percentage of correct values, indexed by Km.
\end{itemize}

we prompt the model with:
\begin{lstlisting}
Please give a complete list of Activating Compound, Commentand Organism of all substrates in the paper. Usually the substrates' tags are numbers or IUPAC names.
1. Output in csv format, write units not in header but in the value like "10.5 µM". Quote the value if it has comma! For example:
```csv
Activating Compound, Substrate, Inhibitor, Km, Comment, Localization, Organism
Cu2+, - , - , -, "at 0.001 mM of the activity without activator", - ,"Homo sapiens"
p-xylene, - , - , - , "11.4 mM, slight activation", - , "Bos taurus"
```
2. If there are multiple tables, concat them. Don't give me reference or using "...", give me complete table!
3. If information is not found in the document, please use '-' to fill in the table.
\end{lstlisting}

The dataset is curated from BRENDA Enzyme Database(https://www.brenda-enzymes.org/index.php). Given the structuring of the initial dataset by Enzyme Commission (EC) numbers, we selectively sourced ten publications from this collection. These chosen works collectively encompass a broad spectrum of enzyme-related data. Simultaneously, they exhibit a variety of presentation styles for essential data categories, including activating compounds, substrates, inhibitors, Michaelis constants (Km), and taxonomic details of the organisms studied. This deliberate selection strategy was employed to ensure a holistic coverage and facilitate a multifaceted examination of enzymatic activities, thereby enriching the depth and breadth of our enzymological inquiry.

\subsubsection{Conclusion}

From the above results, we can see that with the multi-modal inference ability of Uni-SMART, the performance of tasks related to molecule images has been significantly improved.

% \subsection{Biomedical Knowledge Gragh}
\subsection{Biomedical Content Comprehension}

In this chapter, we conduct tests on the Uni-SMART's capability for biomedical information extraction, focusing primarily on testing the model's ability for semantic recognition of knowledge graph triples (\ref{sec:text_mining_task}, \ref{sec:DNER}), relation extraction (\ref{sec:CID}), and the model's ability to perform question-answering based on biomedical literature (\ref{sec:biomedical_understanding}). Our test results indicate that the model can identify complex entities within paragraph texts, extract relationships among recognized entities, and understand complex biomedical paper semantics, extracting intricate information therein.

Through our evaluation, we summarize the capabilities of Uni-SMART in the Biomedicine domain as follows:

\begin{table*}[h]
\centering
\caption{Quantitative evaluation on Biomedicine benchmarks.}
\begin{tabular}{ccccccc}
\toprule
Task                         & \#No. of Literature & Metric & Uni-SMART & GPT-4  \\
\midrule
MedMCQA    & 0 & Accuracy & \textbf{0.73} &  0.7  \\
"Gene-Disease" Association Semantics Recognition    & 250 & Accuracy & 0.936 &  0.928  \\
Compound Entities Recognition     & 1000      & \begin{tabular}{c} Accuracy \\ Cosine-F1 score  \end{tabular}      &  \begin{tabular}{c} 0.988 \\ 0.602  \end{tabular}  &  \begin{tabular}{c} 0.991 \\ 0.356  \end{tabular}  &       \\
Disease Entities Recognition     & 1000      & \begin{tabular}{c} Accuracy \\ Cosine-F1 score  \end{tabular}     & \begin{tabular}{c} 0.977 \\ 0.401  \end{tabular}  &  \begin{tabular}{c} 0.981 \\ 0.345  \end{tabular}  &       \\
Compound-Disease Relation Extraction        & 1000 & \begin{tabular}{c} Accuracy \\ Macro-F1 score  \end{tabular}   & \begin{tabular}{c} 0.750 \\ NaN  \end{tabular} &  \begin{tabular}{c} NaN \\ NaN  \end{tabular}        \\

\bottomrule
\end{tabular}
\label{tab:quantitative-benckmarks-biomedicine}
\end{table*}

\subsubsection{MedMCQA}

MedMCQA is a large-scale, Multiple-Choice Question Answering (MCQA) dataset designed to address real-world medical entrance exam questions. We use the 300 sampled questions from OpenAI's \href{evals}{https://github.com/openai/evals} repository.

\subsubsection{Text mining task for "Gene-Disease" association semantics}
\label{sec:text_mining_task}

Identifying genes associated with diseases aids in understanding the genetic foundation of diseases, thereby providing crucial insights for the prevention, diagnosis, and treatment of diseases. By identifying "gene-disease" pairs, the mechanisms of "gene-disease" associations could be recognized. Large language models can automatically mine these implicit knowledge entries from textual content, potentially offering solutions for the automated processing of health and medical information. In this part, to verify the text mining capabilities of Uni-SMART, we focus on identifying "gene-disease" pairs from texts.


% 数据集描述
% \textcolor{orange}{[Data source: Text mining task for "Gene-Disease" association semantics (GDAS track,  CHIP 2022)]}

This task was retrieved from GDAS track, CHIP 2022. In the vast body of scientific literature, the mechanistic association of "gene-disease" is described through a series of molecular entities such as mutations, genes, and their trigger terms. 

% 示例输入输出

We prompt the model like this:

%% 再确认一下格式是否正确
%% 单引号导致字体格式变了？？
\begin{lstlisting}
You are comparing a submitted answer to an expert answer on a given question. Here is the data:
[BEGIN DATA]
************
[Task]: In this semantic role regconition task, you need to follow 3 steps. First, you need to identify the entities in the text. Entities can be classified into 2 categories--molecular, and trigger word. 'Molecular' includes disease, gene, protein, and enzyme. 'Trigger word' includes 1)Variation(Var), which means DNA, RNA, and mutations in proteins and changes in molecular structure, e.g. 'mutations on the Arg248 and Arg282', 'mutant R282W', 'missense mutations'; 2)Molecular Physiological Activity (MPA), including molecular activity, gene expression and molecular physiological activity, e.g. 'phosphorylation', 'transcription', 'histone methylation', 'bioactivation of cyclophosphamide'; 3)Interaction, molecule-to-molecule or molecule-to-cell connections, e.g. 'bind', 'interaction'; 4)Pathway, e.g. 'Bmp pathway','PI3K pathway'; 5)Cell Physiological Activity (CPA), Activities at or above the cellular level, including cellular reactivity and cell or organ development and growth, e.g. 'T helper cell responses', 'renal development'; 6)Regulation (Reg), a neutral cue word or phrase meaning no loss or gain, e.g. 'resolved in', 'regulated'; 7)Positive Regulation (PosReg), a cue word or phrase that indicates the acquisition of a function, e.g. 'facilitates', 'enhanced', 'increased'; 8)Negative Regulation (NegReg), a clue word or phrase that indicates a loss of function, e.g. 'suppressed', 'decreased', 'inhibited'. Second, you need to identify the semantic role labeling objects, including 'ThemeOf'(from the main thing entity to the current entity) and 'CauseOf'(From the current entity to the Cause entity). Third, please give me tripples that contain entities and semantic role labeling objects(ThemeOf or Causeof).
User: {input}
***
[Submission]: {completion}
***
[Criterion]: conciseness: Does the answer has the same biological entities and relations as the content? (----not this now 2024.2.6-----)
***
[END DATA]
    

\end{lstlisting}

%% 结果作图：
%% 1. gpt3.5-turbo   
% [2024-01-22 15:46:19, 836] [oaieval.py:238] counts/N: 16
% [2024-01-22 15:46:19, 836] [oaieval.py:238] counts/Y: 234
% [2024-01-22 15:46:19, 836] [oaieval.py:238] score: 0.936
%% 2. gpt4-all
% [2024-01-22 16:45:38, 214] [oaieval.py:236] Final report:
% [2024-01-22 16:45:38, 214] [oaieval.py:238] counts/Y: 232
% [2024-01-22 16:45:38, 214] [oaieval.py:238] counts/N: 18
% [2024-01-22 16:45:38, 214] [oaieval.py:238] score: 0.928
% [2024-01-22 16:45:38, 224] [record.py:349] Logged 50 rows of events to /tmp/evallogs/240122075929Z3NXRX4Q_uni_finder/fast/gpt-4-all_semantic_role_recognition.jsonl
% 改变conciseness后再跑一遍：
% [2024-01-24 16:57:31, 820] [oaieval.py:236] Final report:
% [2024-01-24 16:57:31, 820] [oaieval.py:238] counts/Y: 223
% [2024-01-24 16:57:31, 820] [oaieval.py:238] counts/N: 27
% [2024-01-24 16:57:31, 820] [oaieval.py:238] score: 0.892
% [2024-01-24 16:57:31, 831] [record.py:349] Logged 50 rows of events to /tmp/evallogs/240124080705XXLKZGB2_uni_finder/fast/gpt-3.5-turbo_semantic_role_recognition.jsonl
% % 改变类型为fact
% [2024-01-26 14:14:37, 321] [oaieval.py:236] Final report:
% [2024-01-26 14:14:37, 321] [oaieval.py:238] counts/E: 19
% [2024-01-26 14:14:37, 321] [oaieval.py:238] counts/B: 162
% [2024-01-26 14:14:37, 321] [oaieval.py:238] counts/A: 36
% [2024-01-26 14:14:37, 321] [oaieval.py:238] counts/D: 33
% [2024-01-26 14:14:37, 332] [record.py:349] Logged 50 rows of events to /tmp/evallogs/240126054117ESOMVR2M_uni_finder/fa.5-turbo_semantic_role_recognition.jsonl: insert_time=9.796ms
%  改为F1 score计算



%评测指标如何计算？

This Semantic Role Labeling (SRL) task is evaluated using the Macro F1 score,  denoted as $F1_{SRL}$.

Let's assume we have $n$ categories: $\mathrm{C} 1 ,  \ldots . . .,  \mathrm{Ci},  \ldots . . .,  \mathrm{Cn}$.
Precision $\mathrm{Pi}$ is defined as the number of correctly predicted samples in category $\mathrm{Ci}$ divided by the number of samples predicted as category $\mathrm{Ci}$.
Recall $\mathrm{R} i$ is defined as the number of correctly predicted samples in category $\mathrm{Ci}$ divided by the number of true samples in category $\mathrm{Ci}$.

In the Semantic Role Labeling task,  $n=2$.
The performance metric for the Semantic Role Labeling task is defined as:

$$
F1_{SRL}=Macro \ F1=\frac{1}{2} \sum_{i=1}^2 \frac{2 \times Precision_i \times Recall_i}{Precision_i+Recall_i},  \text{ where } i = 1, 2
$$

What should be noted is that, only when all three components (head entity mention,  relation type,  tail entity mention) are predicted correctly,  it is counted as a correct relation prediction. Specifically,  for conditional relations,  only when (condition mention,  condition relation,  (cause mention,  causal relation,  result mention)) are all predicted correctly,  it is counted as a correct prediction.

%评测了什么能力？

%prompt怎么做的, 如何控制模型的输出？



%zero-shot,  few-shot,  zero-shot+cot, few-shot+cot四种实验对比

%评测效果（GPT4, Uni-SMART, Claude）, 表格/图片

% 案例展示, 体现领域能力



\subsubsection{"Compound-Disease" Association Recognition}
% 数据集描述
% 包含从1000条提及化合物-疾病关系的文献

Manually organizing chemical substances, diseases, and their interrelationships is crucial for biomedical research. However, the high cost of this process and the rapid expansion of the number of biomedical literature have posed significant challenges to researchers. Recently, the development of computational technologies capable of automated extraction of chemical-disease relationships (CDR) has received widespread attention, with numerous innovative methods emerging.  The National Institutes of Health (NIH) initiated a project aimed at automating the extraction of CDR from academic literature, involving two core challenges: \textbf{Disease Named Entity Recognition (DNER)} and \textbf{Chemical-Induced Disease (CID) relationship mining}<sup>[3]</sup>. The project established a large annotated text corpus, which includes all chemical substances, diseases, and their interrelationships manually annotated from 1500 PubMed articles. In this section, we will test Uni-SMART's performance on DNER and CID relationship mining, aiming to demonstrate Uni-SMART's ability to accurately extract disease-named entities and chemical-induced disease relationships from literature.

% 示例输入输出

%评测指标如何计算？

\paragraph{TASK 1. Disease Named Entity Recognition (DNER) and Chemical Named Entity Recognition}
\label{sec:DNER}


For the named entity recognition task in this competition,  the $F1\ score$ is used as the evaluation metric,  denoted as $F1_{DNER}$.

Assuming a literature entry contains multiple entities,  for a single literature,  the number of the same entities correctly identified by the model is $True \ Positive$,  the number of unrelated entities incorrectly identified by the model is $False \ Positive$,  and the number of related entities not identified by the model is $False \ Negatives$. Therefore:

% - Precision: Measures the model's precision/accuracy. It is the ratio of correctly identified positive values (true) to all identified positive values. The precision metric shows the number of entities correctly marked.

% $$Precision = \frac{\text{True Positive}}{ \text{True Positive} + \text{False Positive}}$$

% - Recall: Measures the model's ability to predict the actual positive class. It is the ratio of predicted true positives to actual marked results. The recall metric shows the number of entities correctly predicted.

% $$Recall = \frac{\text{True Positive}}{\text{True Positive} + \text{False Negatives}}$$

% - F1 score: The F1 score is the harmonic mean of precision and recall. 

$$ \text{F1 Score} = \frac{2 \times Precision \times Recall }{ Precision + Recall}$$

Assuming the dataset consists of $n$ literature entries,  the performance metric for the entity recognition task is:

$$F1_{NER}=\frac{1}{n} \sum_{i=1}^n \frac{2 \times Precision_i \times Recall_i}{Precision_i+Recall_i}  ,  i=1, 2, \cdots,  n$$

Note: When two entities point to the same semantics,  they are considered a unified entity. Cosine similarity calculated by theWord2Vec algorithm t Po determine whether two entity words point to the same semantics.

We prompt the model like this:

\begin{lstlisting}
You are comparing a submitted answer to an expert answer on a given question. Here is the data:
[BEGIN DATA]
************
[Task]: You are a biologist AI. I'll give you the abstract of the literature. Please identify all the [compound, disease] relations in the abstract, and just give me a list of all relations you recognized.
User: {input}
***
[Submission]: {completion}
***
[Criterion]: NaN?
***
[END DATA]
    

\end{lstlisting}

% [2024-02-06 22:01:05,043] [record.py:371] Final report: {'accuracy': 0.977, 'f1_score': 0.4007019661213162}. Logged to /tmp/evallogs/240206135358VADRQEWH_uni_finder-v1.26_disease_entities_recognition.jsonl
% [2024-02-06 22:01:05,043] [oaieval.py:243] Final report:
% [2024-02-06 22:01:05,043] [oaieval.py:245] accuracy: 0.977
% [2024-02-06 22:01:05,043] [oaieval.py:245] f1_score: 0.4007019661213162

% [2024-02-06 21:46:50,661] [record.py:371] Final report: {'accuracy': 0.981, 'f1_score': 0.34542523094246713}. Logged to /tmp/evallogs/240206133533RYIVZNJK_zhishu/gpt-4-all_disease_entities_recognition.jsonl
% [2024-02-06 21:46:50,662] [oaieval.py:243] Final report:
% [2024-02-06 21:46:50,662] [oaieval.py:245] accuracy: 0.981
% [2024-02-06 21:46:50,662] [oaieval.py:245] f1_score: 0.34542523094246713

% [2024-02-06 22:17:02,058] [record.py:371] Final report: {'accuracy': 0.988, 'f1_score': 0.6017529244372328}. Logged to /tmp/evallogs/240206140930HJ6YL2E2_uni_finder-v1.26_chemical_entities_recognition.jsonl
% [2024-02-06 22:17:02,058] [oaieval.py:243] Final report:
% [2024-02-06 22:17:02,058] [oaieval.py:245] accuracy: 0.988
% [2024-02-06 22:17:02,058] [oaieval.py:245] f1_score: 0.6017529244372328

% [2024-02-06 22:58:00,698] [record.py:371] Final report: {'accuracy': 0.991, 'f1_score': 0.35304034662863126}. Logged to /tmp/evallogs/240206143623KUCMZ4GR_zhishu/gpt-4-all_chemical_entities_recognition.jsonl
% [2024-02-06 22:58:00,698] [oaieval.py:243] Final report:
% [2024-02-06 22:58:00,698] [oaieval.py:245] accuracy: 0.991
% [2024-02-06 22:58:00,698] [oaieval.py:245] f1_score: 0.35304034662863126
 

\paragraph{TASK 2. Chemical-Induced Disease (CID) Relationship Mining}
\label{sec:CID}

% [TODO]串联 @lyg

The Chemical-Induced Disease (CID) Relationship Mining task is evaluated using the Macro F1 score, denoted as $F1_{CID}$.
Let's assume there are $n$ categories of relations: $\mathrm{C} 1 , \ldots . . ., \mathrm{Ci}, \ldots . . ., \mathrm{Cn}$.
Precision $\mathrm{Pi}$ is defined as the number of correctly predicted samples in category $\mathrm{Ci}$ divided by the number of samples predicted as category $\mathrm{Ci}$.
Recall $\mathrm{R} i$ is defined as the number of correctly predicted samples in category $\mathrm{Ci}$ divided by the number of true samples in category $\mathrm{Ci}$.

The performance metric for the Relation Extraction task is defined as:

$$
F1_{CID}=Macro \ F1=\frac{1}{n} \sum_{i=1}^n \frac{2 \times Precision_i \times Recall_i}{Precision_i+Recall_i}, \text{ where } i = 1,2,\cdots,n
$$

Note: Only when all three components (head entity mention, relation type, tail entity mention) are predicted correctly, it is counted as a correct relation prediction. Specifically, for conditional relations, only when (condition mention, condition relation, (cause mention, causal relation, result mention)) are all predicted correctly, it is counted as a correct prediction.

We prompt the model like this:

\begin{lstlisting}
You are comparing a submitted answer to an expert answer on a given question. Here is the data:
[BEGIN DATA]
************
[Task]: You are a biologist AI. I'll give you the abstract of literature. Please identify all the disease entities in the abstract, and just give me a list of the disease entities you recognized."
User: {input}
***
[Submission]: {completion}
***
[Criterion]: NaN?
***
[END DATA]
    

\end{lstlisting}

%评测了什么能力？

%prompt怎么做的, 如何控制模型的输出？

%zero-shot,  few-shot,  zero-shot+cot, few-shot+cot四种实验对比

%评测效果（GPT4, Uni-SMART, Claude）, 表格/图片



% 案例展示, 体现领域能力

\subsubsection{Understanding biomedical literature}
\label{sec:biomedical_understanding}

Reading and extracting information from biomedical literature is crucial,  as it provides the foundation for understanding the complexities and advancements within the biomedical field. Gender differences play a significant role in the functionality of organs and tissues,  with variations in gene expression and regulatory networks potentially leading to sex-specific therapeutic responses in diseases. Therefore,  we utilize the literature \cite{LopesRamos2020SexDI} as a case study to test the Uni-SMART's capability in reading biomedical literature. This approach allows us to assess the model's ability to navigate complex scientific texts and extract pertinent information,  highlighting its potential in supporting gender-specific biomedical research and therapy development.

% We prompt the model with:
% % [TODO]需要补充文献阅读（也就是Finder）的prompt.

Article Summary Case: When reading a biology paper,  quickly grasping its core viewpoints and main findings is essential. Uni-SMART can swiftly provide a refined summary of the article,  condensing lengthy papers into core information,  aiding readers in quickly understanding research highlights and key conclusions.

\begin{lstlisting}
[Prompt] 
"Please summarize the main research content and findings of this article."
[Uni-SMART]
The main research content of this article involves the investigation of sex differences in gene expression and regulatory networks across 29 human tissues. The study utilized 8,279 whole-genome expression profiles from the Genotype-Tissue Expression (GTEx) project to construct sample-specific gene regulatory networks in healthy human tissues.

Key findings of the study include:

1. Sex-biased regulatory network structures were found in each of the 29 tissues examined.
2. Most transcription factors (TFs) are not differentially expressed between males and females, but many exhibit sex-biased regulatory targeting patterns.
3. Genes that are differentially targeted by TFs are associated with the specific functions of each tissue and with diseases that are specific to that tissue.
4. The study identified significant sex differences in gene regulation across all tissues analyzed, with TFs showing sex-biased targeting patterns.
5. Sex-biased target genes are enriched for tissue-related functions and diseases.
6. The research provides a rich public resource that includes the gene regulatory networks of the 29 tissues.

Overall, the study underscores the importance of considering sex differences in gene regulation to understand health and disease manifestations that are specific to males or females. It also highlights the potential for sex-specific therapeutic responses based on these regulatory differences.
\end{lstlisting}


Entity Recognition Case: Uni-SMART excels at identifying key biological concepts within literature,  enabling a clear understanding of the discussed entities.

\begin{lstlisting}
[Prompt] 
"Please extract the cell-type marker genes described in this article."
[Uni-SMART]
The cell-type marker genes described in the article are as follows:

1. FASN (adipocytes)
2. CDH1 and CLDN7 (epithelial cells)
3. AFP (hepatocytes)
4. KRT10 (keratinocytes)
5. MYH7, TNNI1, and MYOG (myocytes)
6. GAD1 (neurons)
7. STX3 (neutrophils)

These marker genes were not differentially expressed between males and females, except for CDH1 and CLDN7, which showed higher expression in tissues from males, and FASN, which demonstrated higher expression in tissues from females.
\end{lstlisting}

Tool and Algorithm Extraction Case: Uni-SMART not only identifies and extracts key biological concepts from the literature but also accurately captures the important tools and algorithms used by the authors. This means that the techniques and tools used in experimental methods or data analysis processes are made clear,  enhancing comprehension of the applied methodologies.
\begin{lstlisting}
[Prompt]  
"Summarize and describe the bioinformatics tools and algorithms used to obtain the main conclusions in this article."
[Uni-SMART] 
The bioinformatics tools and algorithms used in the study to obtain the main conclusions include:

PANDA (Passing Attributes between Networks for Data Assimilation): This algorithm was used to infer and estimate population-based gene regulatory networks by integrating transcription factor binding motifs, gene expression profiles from the GTEx project, and protein-protein interactions from the StringDB database. PANDA produces a directed network of transcription factors to their target genes.

LIONESS (Linear Interpolation to Obtain Network Estimates for Single Samples): LIONESS was employed to estimate individual gene regulatory networks for each sample in the population. This approach produced 8,279 networks, one for each RNA-seq transcriptome from the GTEx research subjects. LIONESS uses an iterative process that leaves out each individual in a population, estimates the network with and without that individual, and then interpolates edge weights to derive an estimate for the network active in that single individual.

YARN (Yet Another RNA Normalization): This software pipeline was used for quality control, gene filtering, and normalization of the GTEx RNA-seq data to make gene expression levels comparable between tissues while preserving information regarding tissue-specific expression.

limma (Linear Models for Microarray Data): limma was utilized for differential expression analysis. It applies linear modeling and empirical Bayes methods to assess differential expression of genes between males and females across different tissues.

GSEA (Gene Set Enrichment Analysis): GSEA was used to identify sex-biased enrichment of Gene Ontology (GO) terms in each tissue. This method ranks genes based on their differential expression and identifies whether sets of genes associated with particular biological processes are overrepresented at the top or bottom of the ranked list.

MSigDB (Molecular Signatures Database): This database provided the gene sets used for enrichment analysis, including GO terms and KEGG (Kyoto Encyclopedia of Genes and Genomes) pathways.

These tools and algorithms were integral in analyzing the large-scale gene expression data, constructing gene regulatory networks, and identifying sex-biased patterns of gene regulation across human tissues. The combination of these computational methods allowed the researchers to draw conclusions about the molecular basis of sex differences in gene regulation and their association with tissue-specific functions and diseases.
\end{lstlisting}


Article Understanding Case: For those terms and complex details that are difficult to understand,  Uni-SMART provides thorough explanations. It acts like an expert on standby,  helping to clarify the meanings of each technical term and grasp the key points of each conclusion.

\begin{lstlisting}
[Prompt] 
"Based on the content of the literature, discuss the role of transcription factors in gender differences in gene regulation, focusing on the transcription factor MAZ and its differential targeting patterns, and provide reference paragraphs from the main text."
[Uni-SMART]
Transcription factors (TFs) play a crucial role in gender differences in gene regulation by differentially targeting genes in a sex-specific manner. Although most TFs are not differentially expressed between males and females, they can exhibit sex-biased regulatory targeting patterns, meaning that the same TF may regulate different sets of genes in males compared to females. This differential targeting can contribute to the observed sex differences in gene expression and may influence tissue-specific functions and disease susceptibility.

The transcription factor MAZ (MYC-associated zinc finger protein) is highlighted in the study as an example of a TF with differential targeting patterns between males and females. MAZ is ubiquitously expressed and has a wide range of target genes, implicating it in various cellular processes, including development and disease. The study found that MAZ exhibits sex-biased regulatory patterns across many tissues, which could have implications for understanding sex-specific biology and disease.

Reference paragraphs from the main text that discuss the role of TFs in gender differences in gene regulation, with a focus on MAZ, include:

An Example of Differential Targeting by the TF MAZ:
"We found sex-biased regulatory network structures across many tissues, as illustrated by a high number of genes that are differentially targeted between males and females. To characterize how TFs might drive these regulatory sex differences, we evaluated how TF targeting patterns correlate with the expression of their target genes and associate with biological pathways. [...] The motif for MAZ, MYC-associated zinc finger protein, was significantly enriched across many tissues (Table S7). MAZ, which encodes a zinc finger TF, is ubiquitously expressed and has 13,270 target genes (genes with the TF binding motif in the promoter region). Thus, MAZ is involved in many cellular processes, including urogenital (Haller et al., 2018), neuronal (Goldie et al., 2017), and tumor development (Cogo et al., 2013; Luo et al., 2016; Yu et al., 2017)."

Differential Targeting by the TF MAZ in Brain (Basal Ganglia):
"We investigated the regulatory role of MAZ in brain (basal ganglia) because this tissue had the third-largest number of differentially expressed genes. To evaluate the regulatory potential of MAZ on its target genes, we started by choosing the autosomal target gene with the highest differential expression in female (PRSS3OP) and the one in male (FRG1B). [...] For both genes, we observed that the weight of the edge from MAZ was linearly correlated with the gene's expression (R²=0.77 for PRSS3OP and R²=0.52 for FRG1B, Figure 4C). MAZ was not differentially expressed between males and females, and its expression was not correlated with the expression of either PRSS3OP or FRG1B (R²=0, Figure 4D)."

These excerpts demonstrate the importance of TFs like MAZ in mediating sex differences in gene regulation. The study's findings suggest that differential targeting by TFs, rather than differences in TF expression levels, may underlie sex-specific regulatory processes in health and disease.

\end{lstlisting}

Assisting Further Exploration Case: Furthermore,  Uni-SMART can summarize issues such as the limitations of an article. Through its understanding of the article's semantics,  it poses questions,  summarizes the literature's limitations,  and inspires new research ideas.
\begin{lstlisting}

[Prompt] 
"Critically evaluate the limitations of this literature (please answer and provide reference paragraphs from the main text), and suggest potential improvements for future research on gene regulation in gender differences."
[Uni-SMART]
The literature acknowledges certain limitations in the study of gene regulation in gender differences, which can be critically evaluated to suggest potential improvements for future research:

1. **Sample Size and Power:**
   "The main limitation of our study is the sample size for some tissues, which might have limited our power to detect sex differences in gene expression and regulatory networks."

   To address this limitation, future research could aim to increase the sample size, particularly for underrepresented tissues, to improve the statistical power and the ability to detect subtle sex differences in gene regulation.

2. **Tissue Heterogeneity:**
   "Another limitation is the tissue heterogeneity, which might have masked cell-type-specific regulatory differences."

   Future studies could improve upon this by employing single-cell sequencing technologies to dissect cell-type-specific regulatory differences, which would provide a more granular understanding of sex differences at the cellular level.

3. **Trans-EQTLs:**
   "We also did not consider trans-eQTLs in our network models, which might have led to an incomplete picture of the regulatory landscape."

   Incorporating trans-eQTLs (expression quantitative trait loci that regulate gene expression at a distance) in network models could provide a more comprehensive view of the regulatory landscape, including long-range genetic effects on gene expression.

4. **X Chromosome Inactivation (XCI):**
   "We also did not consider the XCI status of genes in our analyses, which might have affected our results."

   Future research could take into account the XCI status of genes to refine the understanding of how X-linked gene regulation contributes to sex differences, particularly for genes that escape XCI.

5. **Causal Inference:**
   "Our study is also limited by the correlative nature of the analyses, which does not allow for causal inferences."

   To overcome this limitation, experimental validation of the predicted regulatory interactions and sex differences is necessary. Techniques such as CRISPR-Cas9 gene editing and RNA interference could be used to experimentally manipulate TFs and their targets to establish causality.

6. **Disease Context:**
   "Finally, our study is limited to healthy tissues, and the regulatory networks might be different in the context of disease."

   Expanding the research to include diseased tissues would help to understand how sex differences in gene regulation may change in the context of disease and could inform sex-specific therapeutic strategies.

By addressing these limitations, future research can enhance our understanding of sex differences in gene regulation and their implications for health and disease.

\end{lstlisting}


Knowledge Graph Extraction Case: Uni-SMART is also capable of extracting intuitive knowledge graph information from complex literature,  performing tasks such as entity extraction, relation extraction, and concept hierarchy and classification. This not only shows the connections between concepts but also reveals the network relationships between experimental methods and results,  deepening your understanding of the research field.

\begin{lstlisting}
[Prompt]
"List all the gene names related to gender differences mentioned in the paper."
[Uni-SMART]
The article mentions several genes related to gender differences. Here is a list of gene names that were specifically referenced:

1. MAZ (MYC-associated zinc finger protein)
2. PRSS3OP
3. FRG1B

These genes were discussed in the context of their differential targeting by transcription factors and their potential roles in sex-specific gene regulation. MAZ, in particular, was highlighted for its significant enrichment across many tissues and its involvement in various cellular processes. PRSS3OP and FRG1B were mentioned as examples of autosomal target genes with the highest differential expression in females and males, respectively, in the brain (basal ganglia).

[Prompt]
"Please describe the relationship between gene expression and gender differences mentioned in the text using a series of triplets, and provide reference paragraphs from the main text."
[Uni-SMART]
The relationship between gene expression and gender differences is not explicitly described in the form of triplets in the provided text. However, based on the information given, we can infer some relationships in the form of (Transcription Factor, Target Gene, Gender Difference):

1. (MAZ, PRSS3OP, Higher expression in females)
2. (MAZ, FRG1B, Higher expression in males)

Reference paragraphs from the main text that support these inferred relationships include:

1. **MAZ and PRSS3OP:**
   "To evaluate the regulatory potential of MAZ on its target genes, we started by choosing the autosomal target gene with the highest differential expression in female (PRSS3OP) [...] For both genes, we observed that the weight of the edge from MAZ was linearly correlated with the gene's expression (R²=0.77 for PRSS3OP [...]"

2. **MAZ and FRG1B:**
   "[...] and the one in male (FRG1B). [...] For both genes, we observed that the weight of the edge from MAZ was linearly correlated with the gene's expression (R²=0.52 for FRG1B [...]"

These references indicate that the transcription factor MAZ has a regulatory relationship with the genes PRSS3OP and FRG1B, with PRSS3OP being more highly expressed in females and FRG1B being more highly expressed in males within the brain (basal ganglia) tissue. These relationships exemplify how gene expression can be influenced by gender differences through the differential targeting of transcription factors.

[Prompt]
"Based on the article content, categorize and hierarchize the reasons for differences in gene expression between genders, and provide reference paragraphs from the main text."
[Uni-SMART]
Based on the content of the article, the reasons for differences in gene expression between genders can be categorized and hierarchized as follows:

1. **Differential Targeting by Transcription Factors:**
   The primary reason for differences in gene expression between genders is the differential targeting of genes by transcription factors. The same transcription factor can regulate different sets of genes in males compared to females.
   Reference: "We found sex-biased regulatory network structures across many tissues, as illustrated by a high number of genes that are differentially targeted between males and females."

2. **Sex Chromosome Composition:**
   The presence of different sex chromosomes (XX in females and XY in males) contributes to gene expression differences. This includes the differential expression of genes located on the sex chromosomes and the effects of X chromosome inactivation.
   Reference: "Across all tissues, the median number of differentially targeted genes on the X chromosome was 36 [...] Differentially targeted genes are enriched in escape genes compared with variable escape, inactive, and unknown genes and with autosomes."

3. **Hormonal Influences:**
   Although not explicitly detailed in the provided text, hormonal differences between males and females are known to influence gene expression and could be inferred as a contributing factor to the observed differences in gene regulation.

4. **Tissue-Specific Expression Patterns:**
   Sex differences in gene expression also manifest in tissue-specific patterns, where certain tissues may exhibit more pronounced differences due to the unique functional roles and regulatory environments in males and females.
   Reference: "We found sex-biased regulatory network structures across many tissues [...]"

5. **Biological Pathway and Disease Associations:**
   The differences in gene expression between genders are associated with distinct biological pathways and disease susceptibilities, which can be sex-biased.
   Reference: "We ran pre-ranked GSEA to identify the GO terms and Kyoto Encyclopedia of Genes and Genomes (KEGG) pathways enriched for genes differentially targeted between males and females."

These categories provide a hierarchical framework for understanding the complex interplay of factors that contribute to gender differences in gene expression. The study emphasizes the role of transcription factors and sex chromosomes as primary drivers, with tissue-specific expression patterns and biological pathway associations further shaping the sex-specific regulatory landscape.

\end{lstlisting}

The results show that Uni-SMART achieves excellent effects in understanding literature,  extracting entities,  relationships, attempting concept hierarchy and classification.

% 示例输入输出
%评测指标如何计算？
%评测了什么能力？
%prompt怎么做的, 如何控制模型的输出？
%zero-shot,  few-shot,  zero-shot+cot, few-shot+cot四种实验对比
%评测效果（GPT4, Uni-SMART, Claude）, 表格/图片
% PubMedQA 目前效果不好, 所以改为以上特定文献案例展示
% 数据集描述
% PubMedQA has 1k expert labeled,  61.2k unlabeled and 211.3k artificially generated QA instances.
% PubMedQA
% 1. unifinder-1.26
% [2024-02-04 00:07:40, 492] [oaieval.py:232] Final report:
% [2024-02-04 00:07:40, 493] [oaieval.py:234] accuracy: 0.058823529411764705
% [2024-02-04 00:07:40, 493] [oaieval.py:234] boostrap_std: 0.062211333372625924
% [2024-02-04 00:07:40, 501] [record.py:360] Logged 34 rows of events to /tmp/evallogs/240203160735VKN77JSF_uni_finder-v1.26_pubmedqa.jsonl: insert_time=7.041ms


% 案例展示, 体现领域能力


% \subsection{RE from BioGPT}  %标题是暂定的 %@永歌

% 数据集描述

% 示例输入输出

%评测指标如何计算？

%评测了什么能力？

%prompt怎么做的, 如何控制模型的输出？

%zero-shot,  few-shot,  zero-shot+cot, few-shot+cot四种实验对比

%评测效果（GPT4, Uni-SMART, Claude）, 表格/图片

% 案例展示, 体现领域能力

\subsubsection{Conclusion}

In summary, the Uni-SMART model has demonstrated significant capabilities in handling biomedical tasks, which can be summarized in two key areas:

1. The model exhibits a proficient ability in extracting and recognizing biomedical-related knowledge graphs. It adeptly identifies and extracts complex entities and their interrelationships within biomedical data, showcasing its strength in understanding and processing structured biomedical information. This capability is crucial for advancing research in the biomedical field, as it allows for the effective organization and analysis of vast amounts of data, facilitating the discovery of new insights and the advancement of medical knowledge.

2. Additionally, the Uni-SMART model excels in comprehending complex semantics within biomedical literature and providing assistance in research. It not only understands intricate biomedical paper semantics but also extracts valuable information, demonstrating an advanced level of comprehension that surpasses basic information retrieval. This understanding enables the model to contribute significantly to biomedical research, assisting researchers in navigating through complex literature, synthesizing findings, and answering sophisticated questions that arise during the research process.

These capabilities of the Uni-SMART model underscore its potential as a powerful tool in the biomedical research landscape, offering advanced support in knowledge extraction, semantic understanding, and research assistance.

==> chapters/5_limitations_and_fw.tex <==
\section{Limitations and Future Enhancements}
\label{sec:limitation}
This section delineates the inherent constraints of our work and outlines prospective avenues for advancing Uni-SMART's efficacy and reliability.

\subsection{Acknowledged Limitations}

\textbf{Hallucinations:} Uni-SMART, despite its novel approach to analyzing multimodal scientific literature, is not immune to generating inaccuracies or engaging in flawed reasoning. Such instances of hallucination highlight the importance of critical scrutiny when employing its outputs, especially in situations where precision is paramount. This underscores an ongoing need to enhance the model's accuracy and reliability.

\textbf{Data Quality Concerns:} The performance and output integrity of Uni-SMART are directly influenced by the quality and scope of its training data. Biases, gaps, or inaccuracies in the data can propagate to the model's outputs, potentially compromising the reliability of its analyses and conclusions.

\textbf{Complexity in Evaluation:} Traditional evaluation metrics fall short of capturing the multifaceted nature of scientific text comprehension and generation. Accurately assessing Uni-SMART's performance requires innovative metrics that reflect the complexity and nuance of scientific literature analysis.

\textbf{Grasping Complex Relationships:} The intricate relationships prevalent in scientific discourse pose significant challenges for Uni-SMART. Enhancing its ability to understand and articulate these relationships remains a critical area for development.

\subsection{Vision for Future Enhancements}

\textbf{Counteracting Hallucinations:} Future iterations will focus on bolstering the model's reliability through the integration of robust fact-checking frameworks and the enhancement of its inferential reasoning capabilities. This will involve the adoption of advanced logical inference algorithms and an expansion of the reasoning tasks employed during training.

\textbf{Elevating Data Quality:} We aim to refine the preprocessing and curation of training data to ensure its comprehensiveness and diversity. This includes developing methodologies for identifying and correcting biases or inaccuracies in both the training data and the model's outputs.

\textbf{Innovating Evaluation Metrics:} There is a pressing need for the development of more nuanced evaluation metrics that better encapsulate the intricacies of scientific text analysis. These metrics should evaluate the model's logical reasoning, understanding of complex concepts, and immunity to inaccuracies.

\textbf{Enhanced Understanding of Complex Relationships:} Advancements in relationship extraction techniques will be pursued to improve Uni-SMART's ability to navigate and elucidate the complex interconnections within scientific literature. This will involve specialized training and the integration of external knowledge bases to provide additional contextual insights.


==> chapters/5_risks.tex <==
\section{Risks}
\textcolor{orange}{[Discussion of the potential risks in domains like drug discovery. Need domain expertise.]}


==> chapters/7_contribution.tex <==
\section*{Author Contributions}

\textbf{Linfeng Zhang}: Supervision, Funding acquisition.

\textbf{Guolin Ke}: Supervision, Project administration, Conceptualization, Methodology.

\textbf{Hengxing Cai}: Conceptualization, Methodology, Software, Validation, Writing - Original Draft.

\textbf{Xiaochen Cai}:

\textbf{Junhan Chang}: Software, Validation, Writing - Original Draft.

\textbf{Changxin Wang}: Validation, Writing - Original Draft

\textbf{Zhifeng Gao}: Validation, Writing - Original Draft.

\textbf{Mujie Lin}: Validation, Writing - Original Draft.

\textbf{Yuqi Yin}: Validation, Writing - Original Draft.


{\color{orange}
[Will delete in the future] Choose from following list of contributions. These contributions can include:

\textbf{Conceptualization:} Ideas; formulation or evolution of overarching research goals and aims.

\textbf{Methodology:} Development or design of methodology; creation of models.

\textbf{Software:} Programming, software development; designing computer programs; implementation of the computer code and supporting algorithms.

\textbf{Validation:} Verification, whether as a part of the activity or separate, of the overall replication/reproducibility of results/experiments and other research outputs.

\textbf{Formal analysis:} Application of statistical, mathematical, computational, or other formal techniques to analyze or synthesize study data.

\textbf{Investigation:} Conducting a research and investigation process, specifically performing the experiments, or data/evidence collection.

\textbf{Resources:} Provision of study materials, reagents, materials, patients, laboratory samples, animals, instrumentation, computing resources, or other analysis tools.

\textbf{Data Curation:} Management activities to annotate (produce metadata), scrub data, and maintain research data (including software code, where it is necessary for interpreting the data itself) for initial use and later re-use.

\textbf{Writing - Original Draft:} Preparation, creation, and/or presentation of the published work, specifically writing the initial draft (including substantive translation).

\textbf{Writing - Review:} Preparation, creation, and/or presentation of the published work by those from the original research group, specifically critical review, commentary or revision – including pre- or post-publication stages.

\textbf{Visualization:} Preparation, creation, and/or presentation of the published work, specifically visualization/data presentation.

\textbf{Supervision:} Oversight and leadership responsibility for the research activity planning and execution, including mentorship external to the core team.

\textbf{Project administration:} Management and coordination responsibility for the research activity planning and execution.

\textbf{Funding acquisition:} Acquisition of the financial support for the project leading to this publication.
}
